Extracting associations and meanings of objects depicted in artworks through bi-modal deep networks

We present a novel bi-modal system based on deep networks to address the problem of learning associations and simple meanings of objects depicted in "authored" images, such as fine art paintings and drawings. Our overall system processes both the images and associated texts in order to learn associations between images of individual objects, their identities and the abstract meanings they signify. Unlike past deep nets that describe depicted objects and infer predicates, our system identifies meaning-bearing objects ("signifiers") and their associations ("signifieds") as well as basic overall meanings for target artworks. Our system had precision of 48% and recall of 78% with an F1 metric of 0.6 on a curated set of Dutch vanitas paintings, a genre celebrated for its concentration on conveying a meaning of great import at the time of their execution. We developed and tested our system on fine art paintings but our general methods can be applied to other authored images.

==> Greg/related_work.tex <==
\usepackage[a4paper, total={6in, 8in}]{geometry}
\usepackage[colorlinks=true, urlcolor=blue, citecolor=blue]{hyperref}
\usepackage{dirtytalk}
\usepackage{amsmath,amsfonts,amssymb,amsthm}
\usepackage{mathtools}
\usepackage{relsize}
\usepackage{bm}
\usepackage{adjustbox}
\usepackage{amssymb}
\usepackage{subfigure}
\usepackage{dsfont}
\bibliographystyle{abbrv}

\title{Related Work}

\begin{document}

\maketitle

\section{Knowledge Graph-based Image Captioning}

Previous works sought to generate scene-graphs (include references) and incorporate common-sense knowledge graphs (include references) for downstream tasks such as image captioning.  These methods only deal with the relationships between the objects in the image, as well as the objects and real-world concepts, i.e. bus stop sign and bus station \cite{ImageCaptioningInternalExternalKnowledge}.

However, the 

\bibliography{Art.bib}

\end{document}
